VerifiNER: Verification-augmented NER via Knowledge-grounded Reasoning with Large Language Models

Recent approaches in domain-specific named entity recognition (NER), such as biomedical NER, have shown remarkable advances. However, they still lack of faithfulness, producing erroneous predictions. We assume that knowledge of entities can be useful in verifying the correctness of the predictions. Despite the usefulness of knowledge, resolving such errors with knowledge is nontrivial, since the knowledge itself does not directly indicate the ground-truth label. To this end, we propose VerifiNER, a post-hoc verification framework that identifies errors from existing NER methods using knowledge and revises them into more faithful predictions. Our framework leverages the reasoning abilities of large language models to adequately ground on knowledge and the contextual information in the verification process. We validate effectiveness of VerifiNER through extensive experiments on biomedical datasets. The results suggest that VerifiNER can successfully verify errors from existing models as a model-agnostic approach. Further analyses on out-of-domain and low-resource settings show the usefulness of VerifiNER on real-world applications.

==> 1_intro.tex <==
\section{Introduction}

Named entity recognition (NER) is a fundamental task in natural language processing that aims to identify specific types of entities in given text.
Recent advances in named entity recognition enable its application in diverse domains, such as clinical text and legal text. These approaches show ..., by fine-tuning language models on domain-specific NER datasets.

However, low-resource and cross-domain problems in practical scenarios still pose a great challenge to NER models. Collecting datasets for fine-tuning is not feasible in most practical cases, as it requires annotators with expert-level knowledge in the domains and its accompanying expensive costs. To resolve this issue, more recent work proposes to leverage large language models (LLMs) using their in-conext learning capability \citep{ashok2023promptner, wang2023gptner}. Given a target document and few-shot exemplars, they instruct LLMs to predict entities in an auto-regressive manner, where the output text is a document augmented with special tokens (e.g., ``\texttt{\#\#}'', ``\texttt{@@}'', and ``\texttt{<C>}'') to denote the predicted entities. 

NER models, whether it be fine-tuning or LLM, tend to hallucinate and output incorrect answers. Specific types of hallucinations in NER task can be classified into five types: 
\textbf{Label error} occurs when the entity is predicted with wrong label. 
\textbf{Span error} occurs when the span of entity is misaligned with gold entity. 
\textbf{Label and Span error} The three error types can also be described as overlapping false positive cases. While the aforementioned three errors somehow overlap with gold annotation, remaining two errors are completely wrong predictions. \textbf{Spurious error} An entity is predicted by the NER model, but is not annotated in the hand-labelled text. Complete false positive case. 

\textbf{Missing error} occurs when the model fails to predict targeted entity. The error is also known as false negative case. However, as this work concerns with positive cases, missing error is not in the scope of our concern. 




Despite their potential, we find LLMs have limitations in identifying entities correctly which originated from their limited knowledge. While these models are trained on vast amounts of text from diverse domains, they do not possess an expert-level understanding of specialized fields. Consequently, their performance on domain-specific NER tasks tends to be sub-optimal, as they struggle to capture the jargons and phrasal structures specific to those domains. Incorporating non-parametric, external knowledge such as knowledge base helps address these issues stemming from reliance on LMs' parametric knowledge \citep{mallen-etal-2023-trust}. External knowledge works as an evidence to determine whether prediction from NER models is correct or wrong. 




While knowledge bases (KB) contain vast repositories of domain-specific and factual information, they are organized in a standardized format, thus making it difficult to adapt in real-world settings.  Simply appending knowledge, or manually programming to align knowledge with predicted output is not fully leveraging rich informativity of knowledge base, nor exploiting reasoning ability of LLMs. 

To resolve the issue, we introduce a verification method for NER systems that can improve insufficient and incorrect knowledge of LLMs by incorporating knowledge bases (KB). To better leverage the knowledge provided by KBs, (method)

To our knowledge, our work is the first to verify model-agnostic NER outputs while incorporating external knowledge as evidence. Our work is able to verify any formats or kinds of NER outputs, from whichever model used beforehand. We perform experiments on three biomedical NER datasets with both fine-tuned models and large language models. ... (results)

Our contributions are as follows:
\begin{itemize}
    \item We introduce a novel task of named entity verification
    \item We present a \textbf{\textsc{nerve}} framework.
    \item Our results show ...
\end{itemize}

% 주안점을 어디에 둘건지??
% 1. KB) knowledge base를 LLM을 활용해서 손쉽게 사용할 수 있다
% 2. Verification) NER에 verification 적용한게 처음이다

\begin{comment}
% ver. 231227
Named entity recognition (NER) is a fundamental task in natural language processing that aims to identify specific types of entities in given text.
Recent advances in named entity recognition enable its application in diverse domains, such as clinical text and legal text. These approaches show ..., by fine-tuning language models on domain-specific NER datasets.

However, challenges of such models lie in that \textbf{1} fine-tuning models do not have capability to interpret its own output, as it does not contain knowledge and merely recognize entities from pattern, and \textbf{2} they still fail to reach completely reliable and accurate performance. They tend to output incorrect answers, or "hallucinate". In specific, hallucinations in NER task can be categorized into five types. 

\textbf{Label error} occurs when the entity is predicted with wrong label. 
\textbf{Span error} occurs when the span of entity is misaligned with gold entity. 
\textbf{Label and Span error} is two errors combined. The three error types can also be described as overlapping false positive cases. While the aforementioned three errors somehow overlap with gold annotation, remaining two errors are completely wrong predictions. \textbf{Spurious error} An entity is predicted by the NER model, but is not annotated in the hand-labelled text. Complete false positive case. \textbf{Missing error} occurs when the model fails to predict targeted entity. The error is also known as false negative case. However, as this work concerns with positive cases, missing error is not in the scope of our concern. 

Such errors can be mitigated by utilizing knowledge base as source. Knowledge base has its benefit in factual and reliable knowledge. (blablabla kb)

Suppose we are using fine-tuned NER models and trying to verify its output. We look up dictionaries and reliable sources to obtain evidence and knowledge for determining whether the prediction is correct or not. Similarly, we attempt to imitate human cognitive process of verifying outputs from fine-tuned models, by leveraging reasoning ability of LLM. 

LLM blababab (good performance, able to instruction tuning blab)


We propose a novel task of NER verification. In specific, we test our framework in biomedical datasets, because biomedical domain is knowledge-intensive and thus able to benefit from using KB. 

We use 

\end{comment}

Recent works have proposed LM augmentation with external knowledge (Baek et al., 2023), or knowledge-grounded verification (Zhao et al, 2023) to mitigate hallucination and ensure factual consistency of the model. However, most works deal with QA task, as QA task is knowledge-intensive and prone to hallucinations. We believe other NLP tasks besides QA can also be subject for verification. For instance, named entity recognition (NER) task is also knowledge -intensive and offer room for verification. Typical categories of hallucinations, or error types can be classified into five. (Section 2)
For mitigating hallucination in NER, external knowledge is required 






==> figure_latex/case_study.tex <==
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/combo_examples_1.pdf}
\caption{
An example of a QA pair and the passage matching results by \model. 
}
\label{fig:combo_examples}
\end{figure}



==> figure_latex/error_type.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/error_analysis.png}
    \caption{Error analysis. (temporary figure)}
    \label{fig:error_analysis} 
\end{figure} 

==> figure_latex/figure1_new.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\columnwidth]{figures/figure1_new.png}
    \caption{Motivating example of importance of external knowledge in NER. (temporary figure)}
    \label{fig:error} 
\end{figure} 

==> figure_latex/prompt.tex <==
\begin{figure}[!ht]
\begin{tcolorbox}[colback=gray!4!white,colframe=gray!80!black,fonttitle=\bfseries, title=Knowledge Verbalizer Prompt]
% \begin{equation}
    \begin{minipage}[!ht]{\linewidth}
    \textit{The definition of \{$\Tilde{\textbf{s}}_{ij}$\} is \{definition\}.}\\
    \textit{The semantic type of \{$\Tilde{\textbf{s}}_{ij}$\} is \{semantic\_type\}}.
    \end{minipage}
% \end{equation}
\end{tcolorbox}
\caption{Knowledge verbalizer prompt for generating knowledge-grounded evidence.}
    \label{fig:verb_prompt}
\end{figure}

==> tables/bio_table.tex <==
\begin{table*}[ht]
\small
\centering
\begin{tabular}{lcccccc}
\toprule
 &
  \multicolumn{3}{c}{\textbf{BC5CDR}} &
  \multicolumn{3}{c}{\textbf{GENIA}} \\ 
  \cmidrule(lr){2-4} \cmidrule(l){5-7}
  
% \textbf{Models} & 
\textbf{} & 
  Precision &
  Recall &
  F1 &
  Precision &
  Recall &
  F1 \\ 
\toprule

\textsc{GPT-NER} & 75.44 & 45.74 & 56.95 & 56.83 & 36.2 & 44.23 \\ 
\hspace{0.1cm}+ LLM-verification & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & - & - & - \\
\hspace{0.1cm}\textbf{+ \textsc{nerve} (Ours)} & \textbf{78.78} & \textbf{50.2} & \textbf{61.32} & \textbf{62.06} & \textbf{41.18} & \textbf{49.5} \\ \midrule

\textsc{ConNER} & 89.48 & 92.22 & 90.83 & 77.07 & 84.53 & 80.63 \\ 
\hspace{0.1cm}+ LLM-verification & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & - & - & - \\
\hspace{0.1cm}\textbf{+ \textsc{nerve} (Ours)} & 87.9 & 91.62 & 89.72 & 72.49 & 83.79 & 77.73 \\ \midrule

\textsc{BioBERT} & 63.77 & 75.43 & 69.11 & 53.96 & 47.42 & 50.48 \\ 
\hspace{0.1cm}+ LLM-verification & - & - & - & - & - & - \\
\hspace{0.1cm}+ LLM-verification \& CoT & - & - & - & - & - & - \\
\hspace{0.1cm}\textbf{+ \textsc{nerve} (Ours)} & \textbf{70.08} & \textbf{79.25} & \textbf{74.39} & \textbf{62.55} & \textbf{56.68} & \textbf{59.47} \\ 

\bottomrule

\end{tabular}
\caption{Main experimental results of our \textsc{nerve} and compared approaches. Evaluation is done on token-level.}
\label{tab:bio_results}
\end{table*}

==> tables/cross_dataset.tex <==


\begin{table*}[!ht]
% \small
\centering
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
% \multirow{2}{*}{Source $\to$ Target}
\multirow{2}{*}{Source $\to$ Target}
 &
  \multicolumn{3}{c}{\textbf{GENIA} $\to$ \textbf{BC5CDR}} &
  \multicolumn{3}{c}{\textbf{BC5CDR} $\to$ \textbf{GENIA}} \\ 
  \cmidrule(lr){2-4} \cmidrule(l){5-7}

  
% \textbf{Models} & 
\textbf{} & 
  P &
  R &
  F &
  P &
  R & 
  F \\ 
\toprule
\rowcolor{defaultcolor} \textsc{ConNER} (on Target) & 85.67 & 96.47 & 90.75 & 74.13 & 96.69 & 83.92 \\ \midrule
\textsc{ConNER} (unseen) & N/A & N/A & N/A & N/A & N/A & N/A  \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & \textbf{76.74} & \textbf{57.42} & \textbf{65.69} & \textbf{58.15} & \textbf{77.42} & \textbf{66.42} \\ \midrule\midrule

\rowcolor{defaultcolor} \textsc{BioBERT} (on Target) & 63.87 & 76.06 & 69.44 & 54.51 & 65.30 & 59.42 \\ \midrule
\textsc{BioBERT} (unseen) & N/A & N/A & N/A & N/A & N/A & N/A \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & \textbf{77.64} & \textbf{71.17} & \textbf{74.27} & \textbf{66.49} & \textbf{87.25} & \textbf{75.47} \\ \midrule\midrule


\rowcolor{defaultcolor} \textsc{GPT-NER} & 79.84 & 47.48 & 59.55 & 56.44 & 42.15 & 48.26 \\ 

\bottomrule

\end{tabular}
}
\caption{Experimental results on unseen settings. Evaluation is done on entity-level.}
\label{tab:cross_dataset_results}
\end{table*}

==> tables/error_types_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\newcolumntype{C}{>{\centering\arraybackslash}p{0.1\columnwidth}}
\newcolumntype{R}{>{\raggedleft\arraybackslash}p{0.1\columnwidth}}
\newcolumntype{L}{>{\raggedright\arraybackslash}p{0.35\textwidth}}
% \newcolumntype{L1}{>{\raggedright\arraybackslash}p{0.1\textwidth}}
\newcolumntype{F}{>{\raggedright\arraybackslash}p{0.55\textwidth}}

\begin{table*}[!ht]
\centering
\small
\renewcommand{\tabcolsep}{1mm}
\resizebox{.99\textwidth}{!}{
\begin{tabular}{ccLl}
\toprule
% \multicolumn{4}{l}{\textbf{Gold annotation}}\\
\multicolumn{4}{l}{
\multirow{2}{*}{
\textbf{Gold annotation:} ``… cell adhesion to cytokine-stimulated ${\underset{\textcolor{green}{\textbf{\texttt{cell\_type}}}}{\textcolor{green}{\textbf{\text{[endothelial cells]}}}}}$ by ..''
}
}\\\\
\toprule
& \textbf{Error type}& \multicolumn{1}{c}{\textbf{Definition}} & \multicolumn{1}{c}{\textbf{Example}}\\
\midrule
\renewcommand{\arraystretch}{1.2}
\multicolumn{1}{c}{\multirow{9}{*}{\rotatebox[origin=c]{90}{FP}}} & Type & Wrong type is assigned to an entity & \begin{tabular}[c]{@{}l@{}}
    % \textbf{Context:} 
    ``… cell adhesion to cytokine-stimulated $\underset{\textcolor{red}{\textbf{\texttt{cell\_line}}}}{\textcolor{green}{\textbf{\text{[endothelial cells]}}}}$ by ..'' \\ 
    % \textbf{Pred:} ()\\ 
    % \textbf{Gold:} (endothelial cells, cell\_type)
    \end{tabular}   \\
    \cmidrule{2-4}
    
& \multirow{2}{*}{Span}                 &  Predicted span partially overlaps with ground truth, but incorrect                             & \begin{tabular}[c]{@{}l@{}}
    % \textbf{Context:} 
    ``… cell adhesion to $\underset{\textcolor{green}{\textbf{\texttt{cell\_type}}}}{\textcolor{red}{\textbf{\text{[cytokine-stimulated endothelial cells]}}}}$ by ..'' \\ 
    % \textbf{Pred:} ()\\ 
    % \textbf{Gold:} ()
    \end{tabular}   \\
    \cmidrule{2-4}
    
& {\footnotesize Type\&Span}               & Both type and span are predicted incorrectly                                 & \begin{tabular}[c]{@{}l@{}}
    % \textbf{Context:} 
    ``… cell adhesion to $\textcolor{red}{\underset{\textbf{\texttt{cell\_line}}}{\textbf{\text{[cytokine-stimulated endothelial cells]}}}}$ by ..'' \\ 
    % \textbf{Pred:} ()\\ 
    % \textbf{Gold:} ()
    \end{tabular}   \\
\cmidrule{2-4}
& \multirow{2}{*}{Spurious}             & A completely incorrect entity is predicted where gold annotation does not exist & \begin{tabular}[c]{@{}l@{}}
    % \textbf{Context:} 
    ``… $\textcolor{red}{\underset{\textbf{\texttt{cell\_line}}}{\textbf{\text{[cell adhesion]}}}}$ to cytokine-stimulated endothelial cells by ..'' \\ 
    % \textbf{Pred:} ()\\ 
    % \textbf{Gold:} ()
    \end{tabular}   \\
\midrule

\multirow{2}{*}{\rotatebox[origin=c]{90}{FN}}                          & \multirow{2}{*}{Missing}              & A gold annotation for entity exists but not predicted by a model & \begin{tabular}[c]{@{}l@{}}
    % \textbf{Context:} 
    "… cell adhesion to cytokine-stimulated endothelial cells by .."
    \end{tabular}
    \\ 
    % \textbf{Pred:} ()\\ 
    % \textbf{Gold:} ()

\bottomrule

\end{tabular}
} 
\caption{\textit{Top:} Ground truth span and type of ``endothelial cells''. 
\textit{Bottom:} Definition and examples per error type. \textcolor{green}{Green} denotes ground truth, and \textcolor{red}{red} denotes error in span and/or type.}
\vspace{-7pt}
\label{tab:error_def}
\end{table*}



==> tables/goal.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{cccc}
\toprule

  \multicolumn{2}{c}{\textbf{BC5CDR}} &
  \multicolumn{2}{c}{\textbf{GENIA}} \\ 
  \cmidrule(lr){1-2} \cmidrule(lr){3-4}
  
% \textbf{Models} & 
  TP to TP &
  FP to TP &
  TP to TP &
  FP to TP \\ 
\toprule
 - & - & - & - \\ 
\bottomrule
\end{tabular}
\caption{Goal Maximization on model-orthogonal benchmark.}
\label{tab:goal}
\end{table}

==> tables/intro_tab.tex <==
\begin{table}[!t]
% \small
\centering
\resizebox{1.\columnwidth}{!}{
\begin{tabular}{lccccc|c}
\toprule

\textbf{Models}&
  \textbf{Type} &
  \textbf{Span} & 
  \textbf{T\&S} &
  \textbf{Spurious} & 
  \textbf{Missing} &
  \textbf{Part. FP} \\ 
\toprule


\textsc{ConNER} & 3.08 & 9.31 & 2.42 & 11.06 & 2.54 & 52.13 \\
\textsc{BioBERT} & 1.78 & 25.02 & 2.16 & 16.53 & 28.96 & 38.9 \\
\textsc{GPT-NER} & 5.11 & 14.16 & 5.95 & 18.32 & 77.45 & 20.84 \\

% \toprule

% \toprule

% & $< 2$ & $2-5$ & $> 5$\\ 
% \toprule
% \textsc{ConNER} & 78.62\% & 20.65\% & 0.74\% \\ 
% \textsc{BioBERT} & 84.68\% & 14.89\% & 0.44\% \\
% \textsc{GPT-NER} & 84.41\% & 15.25\% & 0.35\% \\
\bottomrule

\end{tabular}
}
\caption{The ratio of each error type (\%) of NER models on GENIA dataset. \textbf{Part. FP} is the ratio of partial false positive errors (\ie{}, \textit{type}, \textit{span}, \textit{type\&span}) to total errors. We provide model details in Section~\ref{sec:ner_models}.}
\label{tab:intro} 
\end{table}



==> tables/low_resource_dist_shift_table.tex <==
%수정예정
\begin{table*}[ht!]
% \small
\centering
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
% \multirow{2}{*}{Source $\to$ Target}
%\multirow{2}{*}{Source $\to$ Target}
 &
  \multicolumn{3}{c}{\textbf{GENIA} } &
  \multicolumn{3}{c}{\textbf{BC5CDR} } \\ 
  \cmidrule(lr){2-4} \cmidrule(l){5-7}
                    
  
% \textbf{Models} & 
\textbf{} & 
  P &
  R &
  F &
  P &
  R & 
  F \\ 
\toprule

\textsc{ConNER} (subset 1 $\to$ target ) & - & - & - & - & - & - \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\ \midrule
\textsc{ConNER} (subset 2 $\to$ target) & - & - & - & - & - & - \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & - & - & - & - & - & - \\ \midrule
\textsc{ConNER} (10\% $\to$ target) & - & - & - & - & - & - \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & - & - & - & - & - & - \\ \midrule\midrule

\textsc{BioBERT} (subset 1 $\to$ target)  \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} \\ \midrule

\textsc{BioBERT} (subset 2 $\to$ target)  \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)} &  \\ \midrule

\textsc{BioBERT} (10\% $\to$ target)  \\ 
\hspace{0.1cm}\textbf{+ \verifiner~(Ours)}  \\ 


\bottomrule

\end{tabular}
}
\caption{Experimental results on distribution-shift and low-resource settings. Evaluation is done by entity-level.}
\label{tab:cross_dataset_results}
\end{table*}

==> tables/main_table_old.tex <==
\begin{table*}[ht]
\small
\centering
 \resizebox{1.\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
 &
  \multicolumn{3}{c}{\textbf{BC5CDR}} &
  \multicolumn{3}{c}{\textbf{GENIA}} \\ 
  \cmidrule(lr){2-4} \cmidrule(l){5-7}
  
% \textbf{Models} & 
\textbf{} & 
  Precision &
  Recall &
  F1 &
  Precision &
  Recall &
  F1 \\ 
\toprule

\textsc{GPT-NER} & 84.69 & \textbf{52.98} & 65.19 & 56.44 & 42.15 & 48.26 \\ 
\hspace{0.1cm}+ LLM-verification & 49.94 & 21.37 & 29.93 & 36.52 & 69.53 & 47.89\\
\hspace{0.1cm}+ LLM-verification \& CoT & 49.46 & 20.88 & 29.37 & 22.87 & 48.45 & 31.07\\
\hspace{0.1cm}\textbf{+ \nerve~(Ours)} & \textbf{90.53 (\blue{+ 5.84})} & 51.49 (\textcolor{red}{- 1.49}) & \textbf{65.64 (\blue{+ 0.45})} & \textbf{70.85 (\blue{+ 14.41})} & \textbf{45.81 (\blue{+ 3.66})} & \textbf{55.64 (\blue{+ 7.38})} \\ \midrule

\textsc{ConNER} & \textbf{89.32} & \textbf{94.16} & \textbf{91.68} & 77.70 & \textbf{96.54} & 86.10\\ 
\hspace{0.1cm}+ LLM-verification & 48.33 & 27.65 & 35.17 & 47.01 & 99.4 & 63.83 \\
\hspace{0.1cm}+ LLM-verification \& CoT & 53.7 & 31.59 & 39.78 & 30.45 & 85.15 & 44.86 \\
\hspace{0.1cm}\textbf{+ \nerve~(Ours)} & 87.61 (\textcolor{red}{- 1.71}) & 88.23 (\textcolor{red}{- 5.93})& 87.92 (\textcolor{red}{- 3.76}) & \textbf{79.79 (\blue{+ 2.2})} & 94.66 (\textcolor{red}{- 1.88}) & \textbf{86.59 (\blue{+ 0.49})} \\ \midrule

\textsc{BioBERT} & 63.58 & \textbf{75.56} & 69.06 & 54.49 & 63.85 & 58.80 \\ 
\hspace{0.1cm}+ LLM-verification & 29.31 & 22.94 & 25.74 & 35.75 & 85.1 & 50.35 \\
\hspace{0.1cm}+ LLM-verification \& CoT & 36.24 & 28.12 & 31.67 & 23.48 & 66.51 & 34.71 \\
\hspace{0.1cm}\textbf{+ \nerve~(Ours)} & \textbf{81.56 (\blue{+ 17.98})} & 71.74 (\textcolor{red}{- 3.82}) & \textbf{76.34 (\blue{+ 7.28})} & \textbf{77.80 (\blue{+ 23.31})} & \textbf{68.32 (\blue{+ 4.47})} & \textbf{72.75 (\blue{+ 13.95})} \\ 

\bottomrule

\end{tabular}}
\caption{Main experimental results of our \nerve~and compared approaches. Evaluation is done on entity-level.}
\label{tab:main_results}
\end{table*}

==> tables/unseen_2.tex <==
\begin{table*}[!ht]
% \small
\centering
 \resizebox{1.\textwidth}{!}{
% \renewcommand{\tabcolsep}{1.5mm}
\begin{tabular}{llcccccccccccccccccc}
\toprule
&
 \multicolumn{1}{r}{\textbf{Target}}
 &
  \multicolumn{9}{c}{\textbf{GENIA}} &
  \multicolumn{9}{c}{\textbf{BC5CDR}} \\ 
  \cmidrule(lr){3-11} \cmidrule(l){12-20}

% \multicolumn{1}{l}{\textbf{Models}}
&
\multicolumn{1}{r}{\textbf{Source}}
 &
  \multicolumn{3}{c}{G\textsuperscript{\textdagger}} &
  \multicolumn{3}{c}{G\textsuperscript{*}} &
  \multicolumn{3}{c}{B} &
  \multicolumn{3}{c}{B\textsuperscript{\textdagger}} &
  \multicolumn{3}{c}{B\textsuperscript{*}} &
  \multicolumn{3}{c}{G}
  \\ 
  \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} 
  \cmidrule(lr){12-14} \cmidrule(lr){15-17} \cmidrule(l){18-20} 
  
  \multicolumn{2}{l}{\textbf{Models}}
& 
  P &
  R &
  F &
  P &
  R &
  F &
  P &
  R &
  F &
  P &
  R &
  F &
  P &
  R &
  F &
  P &
  R &
  F
   \\ 

\midrule

\rowcolor{defaultcolor} \multicolumn{2}{l}{\textsc{ConNER}} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\multicolumn{2}{l}{\hspace{0.1cm}\textbf{+ \verifiner~(Ours)}} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\midrule

\rowcolor{defaultcolor} \multicolumn{2}{l}{\textsc{BioBERT}} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\multicolumn{2}{l}{\hspace{0.1cm}\textbf{+ \verifiner~(Ours)}} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\midrule \midrule

\multicolumn{2}{l}{\textsc{GPT-NER}} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\

\bottomrule

\end{tabular}}
\caption{Experimental results on cross-domain and distribution shift settings. We use abbreviations to denote datasets. G is GENIA, B is BC5CDR, and \textdagger, * indicates subset 1 and 2 of each dataset, respectively. Evaluation is done on entity-level.}
\label{tab:unseen2}
\end{table*}

==> tables/unseen_shift.tex <==
%수정예정


% \usepackage{array}
% \usepackage{xcolor}
% \usepackage[table]{xcolor}
% \usepackage{makecell}

% \makeatletter

% \newcommand*{\@rowstyle}{}

% \newcommand*{\rowstyle}[1]{% sets the style of the next row
%   \gdef\@rowstyle{#1}%
%   \@rowstyle\ignorespaces%
% }

% \newcolumntype{=}{% resets the row style
%   >{\gdef\@rowstyle{}}%
% }

% \newcolumntype{+}{% adds the current row style to the next column
%   >{\@rowstyle}%
% }

% \makeatother

\begin{table*}[!ht]
% \small
\centering
\resizebox{1.\textwidth}{!}{
\begin{tabular}{lcccccc|cccccccccccc}
\toprule
% \multirow{2}{*}{Source $\to$ Target}
\multirow{2}{*}{Source $\to$ Target}
 &
  \multicolumn{3}{c}{\textbf{G} $\to$ \textbf{B}} &
  \multicolumn{3}{c}{\textbf{B} $\to$ \textbf{G}} & 
  \multicolumn{3}{c}{\textbf{G$^{\prime}_{1}$} $\to$ \textbf{G}} &
  \multicolumn{3}{c}{\textbf{G$^{\prime}_{2}$} $\to$ \textbf{G}} &
  \multicolumn{3}{c}{\textbf{B$^{\prime}_{1}$} $\to$ \textbf{B}} &
  \multicolumn{3}{c}{\textbf{B$^{\prime}_{2}$} $\to$ \textbf{B}} 
   \\ 
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(l){17-19}

  
% \textbf{Models} & 
\textbf{} & 
  P &
  R &
  F &
  P &
  R & 
  F &
  P &
  R &
  F &
  P &
  R & 
  F &
  P &
  R &
  F &
  P &
  R & 
  F
  \\ 
\toprule
\rowstyle{\color{gray}}
 \textsc{ConNER} (on Target) & 84.90 & 96.47 & 90.32 & 74.13 & 96.69 & 83.92 & 74.13 & 96.69 & 83.92& 74.13 & 96.69 & 83.92 & 84.90 & 96.47 & 90.32 & 84.90 & 96.47 & 90.32 \\ \midrule
\textsc{ConNER} (on Source) & N/A & N/A & N/A & N/A & N/A & N/A & 74.38 & 59.57 & 66.16 & 69.97 & 94.10 & 80.26 & 75.73 & 84.85 & 80.03 & 81.46 & 89.47 & 85.28 \\ 
\rowcolor{defaultcolor} \hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & \textbf{76.74} & \textbf{57.42} & \textbf{65.69} & \textbf{58.15} & \textbf{77.42} & \textbf{66.42} & \textbf{78.86} & \textbf{59.8} & \textbf{68.02} & \textbf{74.16} & 90.03 & \textbf{81.48} & \textbf{93.09} & 80.63 & \textbf{86.41} & \textbf{94.28} & 85.42 & \textbf{89.63}\\ \midrule\midrule

\textsc{BioBERT} (on Target) & 79.93 & 95.98 & 87.22 & 54.51 & 65.30 & 59.42 &  54.51 & 65.30 & 59.42 &54.51 & 65.30 & 59.42 & 79.93 & 95.98 & 87.22 & 79.93 & 95.98 & 87.22 \\ \midrule
\textsc{BioBERT} (on Source) & N/A & N/A & N/A & N/A & N/A & N/A & 15.16 & 16.12 & 15.62 & 35.36 & 64.50 & 45.68 & 46.45 & 55.49 & 50.57 & 61.75 & 69.95 & 65.59\\ 
\rowcolor{defaultcolor} \hspace{0.1cm}\textbf{+ \verifiner~(Ours)} & \textbf{77.64} & \textbf{71.17} & \textbf{74.27} & \textbf{66.49} & \textbf{87.25} & \textbf{75.47} & \textbf{78.27} & \textbf{38.77} & \textbf{51.85} & \textbf{78.91} & \textbf{69.68} & \textbf{74.01} & \textbf{93.33} & \textbf{61.92} & \textbf{74.45} & \textbf{94.16} & \textbf{71.65} & \textbf{81.38}\\ 
\midrule\midrule
\textsc{GPT-NER} & 79.84 & 47.48 & 59.55 & 56.44 & 42.15 & 48.26 & 56.44 & 42.15 & 48.26 & 56.44 & 42.15 & 48.26 & 79.84 & 47.48 & 59.55 & 79.84 & 47.48 & 59.55 \\
\bottomrule

\end{tabular}
}
\caption{Experimental results on cross-domain and distribution shift settings. \textbf{G} is GENIA, \textbf{B} is BC5CDR, and 1, 2 indicates subset 1 and 2 of each dataset, respectively.}
\label{tab:unseen_shift}
\end{table*}


